User-Inspired Posterior Network for Recommendation Reason Generation

Recommendation reason generation, aiming at showing the selling points of products for customers, plays a vital role in attracting customers' attention as well as improving user experience. A simple and effective way is to extract keywords directly from the knowledge-base of products, i.e., attributes or title, as the recommendation reason. However, generating recommendation reason from product knowledge doesn't naturally respond to users' interests. Fortunately, on some E-commerce websites, there exists more and more user-generated content (user-content for short), i.e., product question-answering (QA) discussions, which reflect user-cared aspects. Therefore, in this paper, we consider generating the recommendation reason by taking into account not only the product attributes but also the customer-generated product QA discussions. In reality, adequate user-content is only possible for the most popular commodities, whereas large sums of long-tail products or new products cannot gather a sufficient number of user-content. To tackle this problem, we propose a user-inspired multi-source posterior transformer (MSPT), which induces the model reflecting the users' interests with a posterior multiple QA discussions module, and generating recommendation reasons containing the product attributes as well as the user-cared aspects. Experimental results show that our model is superior to traditional generative models. Additionally, the analysis also shows that our model can focus more on the user-cared aspects than baselines.

==> relatedwork.tex <==


%------------------------------------
%-------- Related Work --------------
%------------------------------------
\section{Related Work}

To the best of our knowledge, recommendation reason generation over product title description, attribute words, community question answering is a novel task in the natural language processing field. We are inspired by several closely related tasks, including headline generation, personalized content generation and multi-document summarization tasks, which have been studied extensively in the past decades. 

\subsection{Headline Generation}
Headline generation aims to describe a document by a compact and informative headline with a small amount of words \cite{dorr2003hedge}. Early work has figured out that a purely extractive approach is not suitable to generate headlines \cite{banko2000headline}. This is mainly because the length of the extracted sentence is often larger than the desired headline size. Besides, the useful information is sometimes distributed across the entire document \cite{zhang2019outline}. With the boom of deep learning, the task is formulated as a Seq2Seq learning problem and neural networks are widely applied in this area. \citet{lopyrev2015generating} adopt an encoder-decoder recurrent neural network with attention mechanism to generate news headlines for the Gigaword corpus. \citet{tan2017neural} generate the headline from multiple summaries using a hierarchical attention model for the New York Times corpus. What's more, there are some researchers focus on headline generation in E-commerce scenario, i.e., product title generation. \citet{sun2018multi} propose a multi-source pointer network which encodes not only source title, but also brand name and commodity name. Both \citet{gong2019automatic} and \citet{wang2018multi} apply attention-based neural networks as their models. \citet{gong2019automatic} consider some rich semantic features of long product titles, while \citet{wang2018multi} design a multi-task model and user searching log data as additional knowledge to facilitate the key words extraction from original long titles. \citet{zhang2019multi} utilize not only the long titles but also the multi-modal information (visual images and attribute tags) with a GAN-based model. 



\subsection{Personalized Content Generation}

Personalized content generation has attracted research interest in various domains, e.g., the automatic generation of marketing messages \cite{roy2015automated}, persuasive message \cite{ding2016personalized} and argument generation \cite{carenini2006generating}. With the support of user preferences, the effectiveness has increases. Recently, \citet{krishna2018vocabulary} present a framework for summary generation that takes into consideration the linguistic preferences of the specific audience. As for computer-based research, \citet{reichelt2014talk} show that personalization of learning materials can increase motivation and learning outcomes. \citet{zander2015does} study the effect of personalization on students' attention allocation using some eye-tracking methods, and find that the personalized parts of reading materials are more attractive. In the field of E-commerce, \citet{chen2019towards} incorporate knowledge base into product description generation model that can generate personalized content. \citet{elad2019learning} propose an extractive method to select sentences and then generate personalized product description. \citet{chen2019pog} build a bridge between personalized outfit generation and recommendation by considering both user preferences and individual items. 


\subsection{Multi-document Summarization}
Text summarization techniques are generally divided into two main approaches: extractive and abstractive. Traditional summarization tasks are mainly based on greedy approaches \cite{carbonell1998use,knight2000statistics}, graphic models \cite{erkan2004lexrank, mihalcea2005language} and optimization-based models \cite{mcdonald2007study}. Multi-document summarization is a new sub-task of text summarization and aims to produce summaries from clusters of thematically related documents. Previous solutions include model transfer, i.e., finetuning single-document summarization model for multi-document summarization data \cite{zhang2018adapting,lebanoff2018adapting,baumel2018query}, or unsupervised models and weakly supervised methods \cite{ma2016unsupervised,chu2018unsupervised,angelidis2018summarizing}. Most recently, \citet{liu2019hierarchical} propose a hierarchical transformer that can represent cross-document relationships via an attention mechanism which allows to share information. \citet{fabbri2019multi} combine the pointer-generator network with an integrated Maximal Marginal Relevance (MMR) \cite{carbonell335use} module.


%%%%%%  double-check the following !!! %%%%%%%%
Compared with existing generation tasks, our task needs to summarize information from questions and several corresponding answers which are related to a certain product. These contents are in large scale and consist of different aspects. Our multiple Question-Answer(s) pairs can be regarded as multiple documents based on the same entity, but there are more complex relationships we need to concern, e.g., the relationship among questions, between one question and its answers, and among relevant answers. To the best of our knowledge, This work is the first to explore the generation of recommendation reason generation in the E-commerce field.

% \subsection{Extension of Transformer Network}
% Transformer \cite{vaswani2017attention} was first proposed for machine translation tasks. Due to the effective ability of language modeling and parallel computation, it becomes popular in research field and has been extended to fit in several directions. \citet{miculicich2018document} improve Transformer with hierarchical attention mechanism to represent the previous sentences in document-level machine translation. \citet{zhang2019recosa} integrate Bi-RNN into Transformer to detect relevent context information for dialogue response generation. \citet{li2019incremental} augment multi-head context attention and document attention to facilitate the document-grounded conversation. \citet{dai2019transformer} bring up Transformer-XL that enables learning dependency beyond a fixed length without disrupting temporal coherence. 

% In contrast to their approach, we extend the Transformer encoder with a novel hierarchical framework that can better capture the complex relationships among the questions and answering discussions based on an interaction module.

